Learning to optimize by multi-gradient for multi-objective optimization

The development of artificial intelligence (AI) for science has led to the emergence of learning-based research paradigms, necessitating a compelling reevaluation of the design of multi-objective optimization (MOO) methods. The new generation MOO methods should be rooted in automated learning rather than manual design. In this paper, we introduce a new automatic learning paradigm for optimizing MOO problems, and propose a multi-gradient learning to optimize (ML2O) method, which automatically learns a generator (or mappings) from multiple gradients to update directions. As a learning-based method, ML2O acquires knowledge of local landscapes by leveraging information from the current step and incorporates global experience extracted from historical iteration trajectory data. By introducing a new guarding mechanism, we propose a guarded multi-gradient learning to optimize (GML2O) method, and prove that the iterative sequence generated by GML2O converges to a Pareto critical point. The experimental results demonstrate that our learned optimizer outperforms hand-designed competitors on training multi-task learning (MTL) neural network.

==> 0_Abstract/content.tex <==
\begin{abstract}
The development of artificial intelligence (AI) for science has led to the emergence of learning-based research paradigms, necessitating a compelling reevaluation of the design of multi-objective optimization (MOO) methods. The new generation MOO methods should be rooted in automated learning rather than manual design.
In this paper, we introduce a new automatic learning paradigm for optimizing MOO problems, and propose a multi-gradient learning to optimize (ML2O) method, which automatically learns a generator (or mappings) from multiple gradients to update directions.
As a learning-based method, ML2O acquires knowledge of local landscapes by leveraging information from the current step and incorporates global experience extracted from historical iteration trajectory data.
By introducing a new guarding mechanism, we propose a guarded multi-gradient learning to optimize (GML2O) method, and prove that the iterative sequence generated by GML2O converges to a Pareto critical point.
The experimental results demonstrate that our learned optimizer outperforms hand-designed competitors on training multi-task learning (MTL) neural network.
\end{abstract} 

==> 1_Introduction/content.tex <==
Multi-objective optimization (MOO) is a popular research topic in optimization, where multiple learning objectives are solved simultaneously.
In general, it is usually impossible to find a single solution  satisfying all objectives best at the same time, but a Pareto optimal set, where improvement in some objective function can only be achieved with the cost of an impairment in some other objectives.
MOO problems has gained wide attention in many real-world scenarios such as semantic segmentation \cite{long2015fully}, online advertising models \cite{lin2019pareto} and autonomous driving systems \cite{huang2019apolloscape,lu2019l3}.
The selection of an appropriate optimization method is crucial to effectively address the MOO problem. This is because different objectives may exhibit conflicting behaviors, resulting in gradients pointing in opposite directions. Additionally, the scales of these objective gradients can vary significantly, leading to a dominance of the largest gradient when simply adding them together.
To address the challenge of conflicting objectives, numerous approaches have been extensively investigated.


One of the methods is scalarization \cite{geoffrion1968proper, gass1955computational}, which obtains the optimal solution to a MOO problem by solving one or several parametrized single-objective optimization problems. These methods are commonly referred to as weighting methods, where nonnegative linear combinations of objective functions are minimized \cite{drummond2008choice,johannes1984scalarization}.
These parameters are not known in advance and requires the researcher to make choices based on their understanding of the objective interaction.
However, the effectiveness of this approach relies on the quality of the weight settings, and simple averages are only applicable in non-conflicting objectives with uniform scales.
Therefore, researchers subsequently proposed the adaptive scalarization technique \cite{kendall2018multi}, wherein the parameters of the scalarization are automatically determined during the course of the algorithm to ensure optimization quality.
This type of method is then no longer limited to designing the weights themselves but to designing the method of weight generation.

% 下面讲梯度法
Meanwhile, non-scalarized MOO methods have also garnered significant attention in recent years. One prominent method is the multiple objective gradient manipulation (MOGM)
\cite{sener2018multi, yu2020gradient, chen2018gradnorm}, which adjusts multiple gradients to identify a shared update direction while ensuring all objectives descend simultaneously.
This class of methods can be generalized to a general framework , where the update direction is a weighted combination of multiple gradients \cite{zhou2022convergence}. Within this framework, MOGM methods can be perceived as a way of generating combinatorial weights, where the weights for each iteration step are computed based on information derived from the current step.
Considering that in practical applications, these full-gradient based methods above can bring unacceptable computational costs,  researchers have increasingly turned their attention to MOGM methods in the stochastic case as a more pragmatic and efficient approach.
Given that the stochastic gradient noise in multi-objective scenarios can potentially lead to an update direction completely opposite to the intended one, mitigating the impact of such noise becomes a central focus for these methods.
In order to alleviate the perturbation caused by gradient noise through leveraging historical information, there exist techniques that integrate momentum-like terms into the gradient \cite{fernando2023mitigating} and weighting parameter components \cite{zhou2022convergence} of these methods, respectively.

The MOO methods described above consist of two components. One component determines the update direction of the current step solely based on the instantaneous gradient of the ongoing iteration \cite{sener2018multi, yu2020gradient, chen2018gradnorm}, while the other component incorporates historical information regarding the trajectory of the iteration \cite{fernando2023mitigating, zhou2022convergence}.
In fact, these MOO methods can be viewed as a type of generator (or mapping) for weighted weights, and the direction of the most rapid descent of the weighted combination of the objective function is the direction of the update suggested by the current method.
The commonality among these generators lies in the fact that their generation strategies are manually pre-specified. Thus the efficacy of the update directions heavily relies on the researcher's priori knowledge about the problem.
This gives rise to two limitations: 1) When confronted with complex problems (e.g., non-convex \cite{pardalos2017non}, constrained MOO \cite{drummond2004projected}, etc.) or problems where the explicit form of the objective function cannot be articulated (e.g., multi-task learning (MTL) \cite{zhang2021survey}), the computation involved in designing suitable weights can become exceedingly challenging.
Researcher must take into account both the local and global landscape of the objective function during algorithm design, as failure to do so may result in iterations easily stuck in local minima and yielding undesirable outcomes.
Meanwhile, manually designed methods often contain undetermined hyperparameters, researchers often resort to a trial and error approach to sift through the myriad of potential parameter combinations and identify the optimal solution for the given problem at hand. However, this process is undoubtedly time-consuming and inefficient.
2) The generalizability of algorithm design processes is limited, particularly for scalarization methods. Even a slight alteration in the objective function's form or problem scale is highly likely to result in failure for the weights or weight generators specifically designed for the current MOO problem.
For instance, in the case of problems with similar scales, the average weighted gradient produces updates that tend to align in a consistent descent direction. In the presence of disparate gradient scales, this gradient may be disproportionately influenced by the largest gradient magnitude while disregarding other objectives.
These difficulties are actually attributed to the conflict in objective functions, which makes it hard to design update direction generators. However, some manually designed MOO methods based on weighted combinations have achieved excellent results in some problems, due to the researchers' profound understanding of the problems.

With the rapid advancement of machine learning, artificial intelligence (AI) has surpassed expectations in comprehending informations \cite{gpt_4, vaswani2017attention,dosovitskiy2020image, shu2023learning}.
Due to the fact that the design process of optimization methods can be seen as researchers' understanding of the changes in objective function values, using AI's powerful understanding ability to replace human cognition and generate an optimization method is very attractive.
Designing optimization methods by AI necessitates the transformation of the human-designed process into a learnable problem, and to learn a generator (or mapping) that can effectively determine the update direction based on the gradient of the objective function.
This transformation as a new paradigm has been proposed in the single-objective optimization and has been demonstrated successful applications across various machine learning optimization tasks \cite{wang2019hyperadam,heaton2020safeguarded,lv2017learning,chen2017learning}. This approach is a mathematical embodiment of the ideas of AI for science, and the single-objective case is known as learning to optimize (L2O) \cite{andrychowicz2016learning}.
Inspired by L2O, we can treat each step of the iterative MOO method as a layer of a neural network, and the process of optimizing the MOO problem can be considered as a learnable recurrent neural network that learns a method for generating update directions from meta-data. In this paper, we propose a learnable generator of MOO update directions, called the multi-gradient learning to optimize (ML2O) method.
The iterative process of ML2O is illustrated in Figure \ref{fig:intro}.
This AI-driven process of conceptualizing and generating optimizers can be regarded as a new paradigm for designing MOO methods. Our proposed ML2O method has two advantages:

${ \bullet }$ ML2O replaces human intervention to comprehend the distinctions and interconnections among multiple objective functions by machine learning, relieving researchers from the arduous task of designing a MOO method.

${ \bullet }$ With the capability of neural networks to approximate arbitrary functions, ML2O is no longer constrained to weighted combinations of gradients from conventional methods when learning a generator in the update direction. This presents an opportunity for exploring a larger function space and achieving more intricate mappings.

Morevoer, we provide the convergence analysis of ML2O and propose a guarded multiple gradients learning to optimize (GML2O) method by incorporating the ideal of safeguard \cite{premont2022simple,heaton2020safeguarded}. Considering that safeguard necessitates a convergent method, we develop a stochastic MOO method called dynamic sampling stochastic multiple gradients (DSSMG) method and establish its convergence to a Pareto critical point. Based on DSSMG, we demonstrate that the iterative sequence generated by the GML2O method converges towards a Pareto critical point.
Experimental results on MTL demonstrate that our ML2O possesses the capability to learn an effective direction for minimizing the loss of all tasks, surpassing conventional scalarization and gradient-based methods in terms of final performance. Our generalizability experiments conducted on various optimization step settings, network structure configurations and datasets, further validate the superiority of our approach over manually designed methods by showcasing its exceptional generalization ability. These findings collectively underscore the outstanding performance of ML2O in optimizing MOO problems. This show that our proposed paradigm has potential to provide a promising avenue for future research.

\begin{figure}[h!]
\centering
\includegraphics[scale=0.4]{figs/ML2O_simple.eps}
%\caption{fig1}
\caption{Diagram of ML2O.  $\mathcal{M}$ denotes the learning optimizer, ${F}$ represents the objective function of MOO and $H$ signifies the historical information of the iteration trajectory.}
\label{fig:intro}
\end{figure}

This paper is organized as follows. Section \ref{sec:preliminaries} presents some basic definitions,
notations and some MOO methods. Section \ref{sec:ML2O} formally introduce the structure and methodology of ML2O. We propose GML2O with a guarded criterion and prove convergence of GML2O in Section \ref{sec:gml2o}.
Experimental results of ML2O and GML2O training MTL neural networks are shown in Section \ref{sec:experment}.
Finally, some conclusions are included in the last section of the paper


==> preamble.tex <==
\usepackage{arxiv}


\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage[hidelinks]{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables

\usepackage{mathtools}
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{lipsum}		% Can be removed after putting your text content
\usepackage{graphicx}

\usepackage{amssymb}
\usepackage{pifont}
\usepackage{xcolor}
\usepackage{caption}
\usepackage{multirow}

\usepackage{hyperref}       % hyperlinks
%\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{multicol}
\usepackage{amsmath}
\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage{subfig}


\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}{Lemma}[section]
\newtheorem{remark}{Remark}[section]
\newtheorem{assumption}{Assumption}[section]
\newtheorem{definition}{Definition}[section]
%\newtheorem{proposition}{Proposition}[section]
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Initialize:}}
% \usepackage[colorinlistoftodos,prependcaption,textsize=tiny]{todonotes}


\title{Learning to optimize by multi-gradient \\for multi-objective optimization}

%\date{September 9, 1985}	% Here you can change the date presented in the paper title
\date{} 					% Or removing it

% \author{%
%     \href{https://orcid.org/0000-0002-7624-1850}{\includegraphics[scale=0.06]{media/orcid.pdf}%
%     \hspace{1mm}%
%     Vittorio Mazzia}\\
%     Alexa AI, Amazon\\
%     \texttt{vmazzia@amazon.com} \\
%     \And
%     \href{}{\includegraphics[scale=0.06]{media/orcid.pdf}%
%     \hspace{1mm}%
%     Alessandro Pedrani}\\
%     Alexa AI, Amazon\\
%     \texttt{pedrana@amazon.com} \\
%     \And
%     \href{https://orcid.org/0000-0002-2178-6052}{\includegraphics[scale=0.06]{media/orcid.pdf}%
%     \hspace{1mm}%
%     Andrea Caciolai}\\
%     Alexa AI, Amazon\\
%     \texttt{andccl@amazon.com} \\
%     \AND
%     \href{}{\includegraphics[scale=0.06]{media/orcid.pdf}%
%     \hspace{1mm}%
%     Kay Rottmann}\\
%     Alexa AI, Amazon\\
%     \texttt{krrottm@amazon.com} \\
%     \And
%     \href{}{\includegraphics[scale=0.06]{media/orcid.pdf}%
%     \hspace{1mm}%
%     Davide Bernardi}\\
%     Alexa AI, Amazon\\
%     \texttt{dvdbe@amazon.com} \\
% 	%% examples of more authors
% 	%% \AND
% 	%% Coauthor \\
% 	%% Affiliation \\
% 	%% Address \\
% 	%% \texttt{email} \\
% 	%% \And
% 	%% Coauthor \\
% 	%% Affiliation \\
% 	%% Address \\
% 	%% \texttt{email} \\
% 	%% \And
% 	%% Coauthor \\
% 	%% Affiliation \\
% 	%% Address \\
% 	%% \texttt{email} \\
% }

\author{ {Linxi Yang}\\
	School of Mathematical Sciences\\
	Sichuan University\\
Sichuan China, 610064 \\
	\texttt{leoyanglinxi@gmail.com} \\
	%% examples of more authors
\And
{Xinmin Yang}\\
	National Center for Applied Mathematics in Chongqing\\
	Chongqing Normal University\\
Chongqing China, 401331 \\
	\texttt{xmyang@cqnu.edu.cn} \\
	\And
	{Liping Tang}\thanks{Corresponding author}  \\
	National Center for Applied Mathematics in Chongqing\\
	Chongqing Normal University\\
Chongqing China, 401331 \\
	\texttt{tanglipings@163.com} \\
	%% \AND
	%% Coauthor \\
	%% Affiliation \\
	%% Address \\
	%% \texttt{email} \\
	%% \And
	%% Coauthor \\
	%% Affiliation \\
	%% Address \\
	%% \texttt{email} \\
	%% \And
	%% Coauthor \\
	%% Affiliation \\
	%% Address \\
	%% \texttt{email} \\
}

% Uncomment to remove the date
%\date{}

% Uncomment to override  the `A preprint' in the header
%\renewcommand{\headeright}{Technical Report}
%\renewcommand{\undertitle}{Technical Report}
\renewcommand{\shorttitle}{\textit{arXiv} Template}
\makeatletter
\renewenvironment{description}
               {\list{}{\labelwidth\z@ \itemindent\z@\leftmargin\z@
                        \let\makelabel\descriptionlabel}}
               {\endlist}
\renewcommand\descriptionlabel[1]{\hspace\labelsep
                                \normalfont\bfseries #1}
\makeatother


%%% Add PDF metadata to help others organize their library
%%% Once the PDF is generated, you can check the metadata with
%%% $ pdfinfo template.pdf
\hypersetup{
pdftitle={A template for the arxiv style},
pdfsubject={~},
pdfauthor={~},
pdfkeywords={~},
}

\hypersetup{
    colorlinks=true,
    linkcolor=blue,
    urlcolor=blue,
    citecolor=blue
}

\usepackage{cleveref}

\definecolor{darkgreen}{RGB}{0,100,0} % define a new color called darkgreen
\newcommand{\greencheck}{\textcolor{darkgreen}{\checkmark}}
\newcommand{\redxmark}{\textcolor{red}{\ding{55}}}

\captionsetup[table]{position=below} 
